The first high-redshift changing-look quasars

We report on three redshift $z>2$ quasars with dramatic changes in their C IV emission lines, the first sample of changing-look quasars (CLQs) at high redshift. This is also the first time the changing-look behaviour has been seen in a high-ionisation emission line. SDSS J1205+3422, J1638+2827, and J2228+2201 show interesting behaviour in their observed optical light curves, and subsequent spectroscopy shows significant changes in the C IV broad emission line, with both line collapse and emergence being displayed on rest-frame timescales of $\sim$240-1640 days. These are rapid changes, especially when considering virial black hole mass estimates of $M_{\rm BH} > 10^{9} M_{\odot}$ for all three quasars. Continuum and emission line measurements from the three quasars show changes in the continuum-equivalent width plane with the CLQs seen to be on the edge of the full population distribution, and showing indications of an intrinsic Baldwin effect. We put these observations in context with recent state-change models, and note that even in their observed low-state, the C IV CLQs are generally above $\sim$5\% in Eddington luminosity.

==> Makefile <==

TEXFILE=CIV_CLQs

default: all



bib: 
	bibtex ${TEXFILE}

all :
	pdflatex  ${TEXFILE}
	pdflatex  ${TEXFILE}
	bibtex ${TEXFILE}
	bibtex ${TEXFILE}
	bibtex ${TEXFILE}
	pdflatex  ${TEXFILE}
	pdflatex  ${TEXFILE}
	pdflatex  ${TEXFILE}
#	dvipdf ${TEXFILE}
	rm -f  ${TEXFILE}.aux
#	rm -f  ${TEXFILE}.bbl
	rm -f  ${TEXFILE}.blg
	rm -f  ${TEXFILE}.dvi
	rm -f  ${TEXFILE}.log
	rm -f  ${TEXFILE}.out
	rm -f  ${TEXFILE}.toc
	rm -f  ${TEXFILE}Notes.bib

	open ${TEXFILE}.pdf


clean:
	rm -f \
	${TEXFILE}.dvi \
	${TEXFILE}.ps \
	${TEXFILE}.out \
	${TEXFILE}.aux \
	${TEXFILE}.bbl \
	${TEXFILE}.blg \
	${TEXFILE}.toc \
	${TEXFILE}.log 
#	${TEXFILE}.pdf 


sup:
	pdflatex  ${TEXFILE_TWO}
	pdflatex  ${TEXFILE_TWO}
	bibtex ${TEXFILE_TWO}
	bibtex ${TEXFILE_TWO}
	pdflatex  ${TEXFILE_TWO}
	pdflatex  ${TEXFILE_TWO}
	rm -f  ${TEXFILE_TWO}.aux
	rm -f  ${TEXFILE_TWO}.bbl
	rm -f  ${TEXFILE_TWO}.blg
	rm -f  ${TEXFILE_TWO}.dvi
	rm -f  ${TEXFILE_TWO}.log
	rm -f  ${TEXFILE_TWO}.out
	rm -f  ${TEXFILE_TWO}.toc
	rm -f  ${TEXFILE_TWO}Notes.bib
	open ${TEXFILE_TWO}.pdf



==> arXiv_submission_notes <==
arXiv_submission_notes




Nicholas~P.~Ross, Matthew J. Graham, Giorgio Calderone, K. E. Saavik Ford, Barry McKernan, and Daniel Stern
\\
%%  List of institutions
$^{1}$Institute for Astronomy, University of Edinburgh, Royal Observatory, Blackford Hill, Edinburgh EH9 3HJ, United Kingdom \\
$^{2}$Cahill Center for Astronomy and Astrophysics, California Institute of Technology, Mail Code 249/17, 1200 E California Blvd, Pasadena CA 91125, USA\\
$^{3}$INAF -- Osservatorio Astronomico di Trieste, Via Tiepolo 11, I-34143 Trieste, Italy \\
$^{4}$Department of Science, BMCC, City University of New York, New York, NY 10007, USA \\
$^{5}$Department of Astrophysics, Rose Center for Earth and Space, American Museum of Natural History, Central Park West at 79th Street, NY 10024, USA \\
$^{6}$Graduate Center, City University of New York, 365 5th Avenue, New York, NY 10016, USA\\
$^{7}$Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Drive, Mail Stop 169-221, Pasadena, CA 91109, USA \\

